Quantifying Engagement with Citations on Wikipedia

Wikipedia, the free online encyclopedia that anyone can edit, is one of the most visited sites on the Web and a common source of information for many users. As an encyclopedia, Wikipedia is not a source of original information, but was conceived as a gateway to secondary sources: according to Wikipedia's guidelines, facts must be backed up by reliable sources that reflect the full spectrum of views on the topic. Although citations lie at the very heart of Wikipedia, little is known about how users interact with them. To close this gap, we built client-side instrumentation for logging all interactions with links leading from English Wikipedia articles to cited references during one month, and conducted the first analysis of readers' interaction with citations on Wikipedia. We find that overall engagement with citations is low: about one in 300 page views results in a reference click (0.29% overall; 0.56% on desktop; 0.13% on mobile). Matched observational studies of the factors associated with reference clicking reveal that clicks occur more frequently on shorter pages and on pages of lower quality, suggesting that references are consulted more commonly when Wikipedia itself does not contain the information sought by the user. Moreover, we observe that recent content, open access sources and references about life events (births, deaths, marriages, etc) are particularly popular. Taken together, our findings open the door to a deeper understanding of Wikipedia's role in a global information economy where reliability is ever less certain, and source attribution ever more vital.

==> data_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\resizebox{\columnwidth}{!}{
\begin{tabular}{lp{2cm}p{9.5cm}}
\textit{}        & {\textbf{Event}}       & \textbf{Description} \\\Xhline{2\arrayrulewidth}
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textit{citation events}}} & \textit{refClick}& A click on an external link in the article's reference section.     \\
 & \textit{extClick}& A click on an external link anywhere in the article.  \\
 & \textit{fnClick} & A click on a footnote number to jump to the reference section at the bottom of the article.     \\
 & \textit{fnHover} & A hover over a footnote number, held for more than 1 second.     \\
 & \textit{upClick} & A click from the reference section to the sentence where a reference is cited.     \\\hline
\textit{}   & \textit{pageLoad}& The action of loading and viewing an article page in Wikipedia.     \\
\textit{}        & \textit{}        &         \\
\textit{}        & {\textbf{Property}}    & \textbf{Description} \\\Xhline{2\arrayrulewidth}

%\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{user}}}& \textit{IP}      & The IP of the reader who generated the event (hashed).     \\
% & \textit{User Agent}           & The User Agent of the reader who generated the event.     \\
 & \textit{Session Token}        & A unique identifier for all events coming from the same tab of a reader's browser. \\\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{\textit{page}}}& \textit{Title}   & The title of the Wikipedia article page where the event took place.     \\
 & \textit{Page\_ID}& The ID of the Wikipedia article page where the event took place.     \\
 & \textit{Text Length}          & The length in character of the Wikipedia article page where the event took place.     \\
 & \textit{\# References} & The number of footnotes in the reference section of the Wikipedia article.     \\
 & \textit{Popularity}           & The number of times a $pageLoad$ event happened in the Wikipedia article.     \\
 & \textit{Topics}  & A 44-dimensional feature vector reflecting the distribution of topics for the Wikipedia article, as classified by the ORES \cite{halfaker_interpolating_2017} \emph{drafttopic} model.     \\
 & \textit{Quality} & The quality level of the Wikipedia article, as classified by the ORES \cite{halfaker_interpolating_2017} \emph{article quality} model     \\\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textit{reference}}}        & \textit{URL}     & The URL of the link that generated the event.     \\
 & \textit{Domain}  & The main domain of the URL.     \\
 & \textit{Reference Text}       & The text of the reference which generated the event, as displayed in the reference section.     \\
 & \textit{Sentence Text}        & The text of the article sentence where the reference is cited.   \\
 & \textit{Relative Position}        & The character offset at which the reference is cited in the text, divided by the total number of characters in the article.   \\
\end{tabular}}
\caption{Data collection summary: types of events captured and list of user, page, and reference properties collected.}
\label{tab:data_collection}
%\todo[Bob]{need a caption!}
\end{table}
